IntCoOp: Interpretability-Aware Vision-Language Prompt Tuning

Image-text contrastive models such as CLIP learn transferable and robust representations for zero-shot transfer to a variety of downstream tasks. However, to obtain strong downstream performances, prompts need to be carefully curated, which can be a tedious engineering task. To address the issue of manual prompt engineering, prompt-tuning is used where a set of contextual vectors are learned by leveraging information from the training data. Despite their effectiveness, existing prompt-tuning frameworks often lack interpretability, thus limiting their ability to understand the compositional nature of images. In this work, we first identify that incorporating compositional attributes (e.g., a "green" tree frog) in the design of manual prompts can significantly enhance image-text alignment scores. Building upon this observation, we propose a novel and interpretable prompt-tuning method named IntCoOp, which learns to jointly align attribute-level inductive biases and class embeddings during prompt-tuning. To assess the effectiveness of our approach, we evaluate IntCoOp across two representative tasks in a few-shot learning setup: generalization to novel classes, and unseen domain shifts. Through extensive experiments across 10 downstream datasets on CLIP, we find that introducing attribute-level inductive biases leads to superior performance against state-of-the-art prompt tuning frameworks. Notably, in a 16-shot setup, IntCoOp improves CoOp by 7.35% in average performance across 10 diverse datasets.

==> tables/main_table.tex <==
\newcolumntype{?}{!{\vrule width 1pt}}
\begin{table*}[!htb]
    
    \begin{subtable}{.27\paperwidth}
      \centering
        \caption{Average over 11 datasets}
        \resizebox{0.9\textwidth}{!}{%
        \begin{tabular}{lll?l}
        \toprule
        & Base & Novel & HM \\
        \midrule
        CLIP & 69.34 & 74.22 & 71.70\\
        CoOp~\cite{zhou2022learning} (IJCV) & 82.69 & 63.22 & 71.66 \\
        Co-CoOp~\cite{zhou2022conditional}(CVPR 22) & 80.47 & 71.69 & 75.83 \\
        ProDA~\cite{lu2022prompt} (CVPR 22) & 81.56 & 72.30 & 76.65 \\
        VPT~\cite{jia2022visual} (ECCV 22) & 80.81 & 70.63 & 74.68 \\
        KgCoOp~\cite{yao2023visual} (CVPR 23) & 80.73 & 73.60 & \underline{77.00} \\
        ProGrad~\cite{zhu2023prompt} (ICCV 23) & 82.48 & 70.75 & 76.16 \\
        \midrule
        \rowcolor{COLOR_ZS} \name (Ours) & 81.30 & 73.78 & \textbf{77.35} \\
        \bottomrule
        \end{tabular}%
        }
    \end{subtable}
    \begin{subtable}{.27\paperwidth}
      \centering
        \caption{ImageNet}
        \resizebox{0.9\textwidth}{!}{%
        \begin{tabular}{lll?l}
        \toprule
        & Base & Novel & HM \\
        \midrule
        CLIP & 72.43 & 68.14 & 70.22 \\
        CoOp~\cite{zhou2022learning} (IJCV) & 76.47 & 67.88 & 71.92 \\
        Co-CoOp~\cite{zhou2022conditional}(CVPR 22) & 75.98 & 70.43 & \underline{73.10} \\
        ProDA~\cite{lu2022prompt} (CVPR 22) & 75.40 & 70.23 & 72.72 \\
        VPT~\cite{jia2022visual} (ECCV 22) & 70.93 & 65.90 & 68.32 \\
        KgCoOp~\cite{yao2023visual} (CVPR 23) & 75.83 & 69.96 & 72.78 \\
        ProGrad~\cite{zhu2023prompt} (ICCV 23) & 77.02 & 66.66 & 71.46 \\
        \midrule
        \rowcolor{COLOR_ZS} \name (Ours) & 75.99 & 71.67 & \textbf{73.77} \\
        \bottomrule
        \end{tabular}%
        }
    \end{subtable}
   \begin{subtable}{0.27\paperwidth}
      \centering
        \caption{Caltech-101}
        \resizebox{0.9\textwidth}{!}{%
        \begin{tabular}{lll?l}
        \toprule
        & Base & Novel & HM \\
        \midrule
        CLIP & 96.84 & 94.00 & 95.40 \\
        CoOp~\cite{zhou2022learning} (IJCV) & 98.00 & 89.81 & 93.73 \\
        Co-CoOp~\cite{zhou2022conditional}(CVPR 22) & 97.96 & 93.81 & 95.84 \\
        ProDA~\cite{lu2022prompt} (CVPR 22) & 98.27  & 93.23 & 95.68 \\
        VPT~\cite{jia2022visual} (ECCV 22) & 97.86 & 93.76 & 95.77 \\
        KgCoOp~\cite{yao2023visual} (CVPR 23) & 97.72 & 94.39 & \underline{96.03} \\
        ProGrad~\cite{zhu2023prompt} (ICCV 23) & 98.02 & 93.89 & 95.91 \\
        \midrule
       \rowcolor{COLOR_ZS} \name (Ours) & 97.80 & 94.76 & \textbf{96.25} \\
        \bottomrule
        \end{tabular}%
        }
    \end{subtable}\\ [1ex]
   
   \begin{subtable}{0.27\paperwidth}
      \centering
        \caption{OxfordPets}
        \resizebox{0.9\textwidth}{!}{%
        \begin{tabular}{lll?l}
        \toprule
        & Base & Novel & HM \\
        \midrule
        CLIP & 91.17 & 97.26 & 94.12\\
        CoOp~\cite{zhou2022learning} (IJCV) & 93.67 & 95.29 & 94.47 \\
        Co-CoOp~\cite{zhou2022conditional}(CVPR 22) & 95.20 & 97.69 & 96.43 \\
        ProDA~\cite{lu2022prompt} (CVPR 22) & 95.43 & 97.83 & \underline{96.62} \\
        VPT~\cite{jia2022visual} (ECCV 22) & 94.81 & 96.00 & 95.40 \\
        KgCoOp~\cite{yao2023visual} (CVPR 23) & 94.65 & 97.76 & 96.18 \\
        ProGrad~\cite{zhu2023prompt} (ICCV 23) & 95.07 & 97.63 & 96.33 \\
        \midrule
        \rowcolor{COLOR_ZS} \name (Ours) & 95.32 & 98.20 & \textbf{96.74} \\
        \bottomrule
        \end{tabular}%
        }
    \end{subtable}
    \begin{subtable}{0.27\paperwidth}
      \centering
        \caption{StanfordCars}
        \resizebox{0.9\textwidth}{!}{%
        \begin{tabular}{lll?l}
        \toprule
        & Base & Novel & HM \\
        \midrule
        CLIP & 63.37 & 74.89 & 68.65\\
        CoOp~\cite{zhou2022learning} (IJCV) & 78.12 & 60.40 & 68.13 \\
        Co-CoOp~\cite{zhou2022conditional}(CVPR 22) & 70.49 & 73.59 & 72.01 \\
        ProDA~\cite{lu2022prompt} (CVPR 22) & 74.70 & 71.20 & 72.91 \\
        VPT~\cite{jia2022visual} (ECCV 22) & 72.46 & 73.38 & 72.92 \\
        KgCoOp~\cite{yao2023visual} (CVPR 23) & 71.76 & 75.04 & \underline{73.36} \\
        ProGrad~\cite{zhu2023prompt} (ICCV 23) & 77.68 & 68.63 & 72.88 \\
        \midrule
       \rowcolor{COLOR_ZS} \name (Ours) & 72.04 & 75.32 & \textbf{73.64} \\
        \bottomrule
        \end{tabular}%
        }
    \end{subtable}
    \begin{subtable}{0.27\paperwidth}
      \centering
        \caption{Flowers102}
        \resizebox{0.9\textwidth}{!}{%
        \begin{tabular}{lll?l}
        \toprule
        & Base & Novel & HM \\
        \midrule
        CLIP & 72.08 & 77.80 & 74.83\\
        CoOp~\cite{zhou2022learning} (IJCV) & 97.60 & 59.67 & 74.06 \\
        Co-CoOp~\cite{zhou2022conditional}(CVPR 22) & 94.87 & 71.75 & 81.71 \\
        ProDA~\cite{lu2022prompt} (CVPR 22) & 97.70 & 68.68 & 80.66 \\
        VPT~\cite{jia2022visual} (ECCV 22) & 95.39 & 73.87 & 83.26 \\
        KgCoOp~\cite{yao2023visual} (CVPR 23) & 95.00 & 74.73 & \underline{83.65} \\
        ProGrad~\cite{zhu2023prompt} (ICCV 23) & 95.54 & 71.87 & 82.03 \\
        \midrule
        \rowcolor{COLOR_ZS} \name (Ours) & 95.82 & 74.54 & \textbf{83.85} \\
        \bottomrule
        \end{tabular}%
        }
    \end{subtable} \\ [1ex]
    
  \begin{subtable}{0.27\paperwidth}
      \centering
        \caption{Food101}
        \resizebox{0.9\textwidth}{!}{%
        \begin{tabular}{lll?l}
        \toprule
        & Base & Novel & HM \\
        \midrule
        CLIP & 90.10 & 91.22 & 90.66\\
        CoOp~\cite{zhou2022learning} (IJCV) & 88.33 & 82.26 & 85.19 \\
        Co-CoOp~\cite{zhou2022conditional}(CVPR 22) & 90.70 & 91.29 & 90.99 \\
        ProDA~\cite{lu2022prompt} (CVPR 22) & 90.30 & 88.57 & 89.43 \\
        VPT~\cite{jia2022visual} (ECCV 22) & 89.88 & 87.76 & 88.81 \\
        KgCoOp~\cite{yao2023visual} (CVPR 23) & 90.50 & 91.70 & \underline{91.09} \\
        ProGrad~\cite{zhu2023prompt} (ICCV 23) & 90.37 & 89.59 & 89.98 \\
        \midrule
        \rowcolor{COLOR_ZS} \name (Ours) & 90.45 & 91.99 & \textbf{91.22} \\
        \bottomrule
        \end{tabular}%
        }
    \end{subtable}
  \begin{subtable}{0.27\paperwidth}
      \centering
        \caption{FGVC Aircraft}
        \resizebox{0.9\textwidth}{!}{%
        \begin{tabular}{lll?l}
        \toprule
        & Base & Novel & HM \\
        \midrule
        CLIP & 27.19 & 36.29 & 31.09\\
        CoOp~\cite{zhou2022learning} (IJCV) & 40.44 & 22.30 & 28.75 \\
        Co-CoOp~\cite{zhou2022conditional}(CVPR 22) & 33.41 & 23.71 & 27.74 \\
        ProDA~\cite{lu2022prompt} (CVPR 22) & 36.90 & 34.13 & \textbf{35.46}\\
        VPT~\cite{jia2022visual} (ECCV 22) & 33.10 & 30.49 & 31.74 \\
        KgCoOp~\cite{yao2023visual} (CVPR 23) & 36.21 & 33.55 & 34.83 \\
        ProGrad~\cite{zhu2023prompt} (ICCV 23) & 40.54 & 27.57 & 32.82 \\
        \midrule
       \rowcolor{COLOR_ZS} \name (Ours) & 36.55 & 33.90 & \underline{35.18} \\
        \bottomrule
        \end{tabular}%
        }
    \end{subtable}
   \begin{subtable}{0.27\paperwidth}
      \centering
        \caption{SUN397}
        \resizebox{0.9\textwidth}{!}{%
        \begin{tabular}{lll?l}
        \toprule
        & Base & Novel & HM \\
        \midrule
        CLIP & 69.36 & 75.35 & 72.23\\
        CoOp~\cite{zhou2022learning} (IJCV) & 80.60 & 65.89 & 72.51 \\
        Co-CoOp~\cite{zhou2022conditional}(CVPR 22) & 79.74 & 76.86 & 78.27 \\
        ProDA~\cite{lu2022prompt} (CVPR 22) & 78.67 & 76.93 & 77.79 \\
        VPT~\cite{jia2022visual} (ECCV 22) & 79.66 & 72.68 & 76.01 \\
        KgCoOp~\cite{yao2023visual} (CVPR 23) & 80.29 & 76.53 & \underline{78.36} \\
        ProGrad~\cite{zhu2023prompt} (ICCV 23) & 81.26 & 74.17 & 77.55 \\
        \midrule
       \rowcolor{COLOR_ZS} \name (Ours) & 80.63 & 76.33 & \textbf{78.42} \\
        \bottomrule
        \end{tabular}%
        }
    \end{subtable} \\ [1ex]

 \begin{subtable}{0.27\paperwidth}
      \centering
        \caption{DTD}
        \resizebox{0.9\textwidth}{!}{%
        \begin{tabular}{lll?l}
        \toprule
        & Base & Novel & HM \\
        \midrule
        CLIP & 53.24 & 59.90 & 56.37\\
        CoOp~\cite{zhou2022learning} (IJCV) & 79.44 & 41.18 & 54.24 \\
        Co-CoOp~\cite{zhou2022conditional}(CVPR 22) & 77.01 & 56.00 & 54.24 \\
        ProDA~\cite{lu2022prompt} (CVPR 22) & 80.67 & 56.48 & \textbf{66.44} \\
        VPT~\cite{jia2022visual} (ECCV 22) & 79.15 & 50.76 & 61.85 \\
        KgCoOp~\cite{yao2023visual} (CVPR 23) & 77.55 & 54.99 & \underline{64.35} \\
        ProGrad~\cite{zhu2023prompt} (ICCV 23) & 77.35 & 52.35 & 62.45 \\
        \midrule
        \rowcolor{COLOR_ZS} \name (Ours) & 79.63 & 50.62 & 61.90 \\
        \bottomrule
        \end{tabular}%
        }
    \end{subtable}
  \begin{subtable}{0.27\paperwidth}
      \centering
        \caption{EuroSAT}
        \resizebox{0.9\textwidth}{!}{%
        \begin{tabular}{lll?l}
        \toprule
        & Base & Novel & HM \\
        \midrule
        CLIP & 56.48 & 64.05 & 60.03\\
        CoOp~\cite{zhou2022learning} (IJCV) & 92.19 & 54.74 & 68.69\\
        Co-CoOp~\cite{zhou2022conditional}(CVPR 22) & 87.49 & 60.04 & 71.21 \\
        ProDA~\cite{lu2022prompt} (CVPR 22) & 83.90 & 66.00 & \underline{73.88} \\
        VPT~\cite{jia2022visual} (ECCV 22) & 93.01 & 54.89 & 69.04 \\
        KgCoOp~\cite{yao2023visual} (CVPR 23) & 85.64 & 64.34 & 73.48 \\
        ProGrad~\cite{zhu2023prompt} (ICCV 23) & 90.11 & 60.89 & 72.67 \\
        \midrule
       \rowcolor{COLOR_ZS} \name (Ours) & 86.26 & 68.00 & \textbf{76.05} \\
        \bottomrule
        \end{tabular}%
        }
    \end{subtable}
   \begin{subtable}{0.27\paperwidth}
      \centering
        \caption{UCF101}
        \resizebox{0.9\textwidth}{!}{%
        \begin{tabular}{lll?l}
        \toprule
        & Base & Novel & HM \\
        \midrule
        CLIP & 70.53 & 77.50 & 73.85\\
        CoOp~\cite{zhou2022learning} (IJCV) & 84.69 & 56.05 & 67.46 \\
        Co-CoOp~\cite{zhou2022conditional}(CVPR 22) & 82.33 & 73.45 & 77.64 \\
        ProDA~\cite{lu2022prompt} (CVPR 22) & 85.23 & 71.97 & 78.04 \\
        VPT~\cite{jia2022visual} (ECCV 22) & 82.67 & 74.54 & 78.39 \\
        KgCoOp~\cite{yao2023visual} (CVPR 23) & 82.89 & 76.67 & \underline{79.65} \\
        ProGrad~\cite{zhu2023prompt} (ICCV 23) & 84.33 & 74.94 & 79.35 \\
        \midrule
       \rowcolor{COLOR_ZS} \name (Ours) & 83.76 & 76.42 & \textbf{79.92} \\
        \bottomrule
        \end{tabular}%
        }
    \end{subtable}
    \caption{\small \textbf{Comparison with competitive prompt-tuning methods on base-to-novel generalization}. We observe that \name consistently demonstrates superior performance over existing prompt-tuning methods. HM represents the harmonic mean of the base and novel accuracies. We train all methods with $16$-shots samples from the base classes. We mark the best accuracies in \textbf{bold} and the \underline{underlined} ones indicate the second best.
    }
    \label{tab:main_table}
    \vspace{-0.3cm}
\end{table*}
